TAGPRIME: A Unified Framework for Relational Structure Extraction

Many tasks in natural language processing require the extraction of relationship information for a given condition, such as event argument extraction, relation extraction, and task-oriented semantic parsing. Recent works usually propose sophisticated models for each task independently and pay less attention to the commonality of these tasks and to have a unified framework for all the tasks. In this work, we propose to take a unified view of all these tasks and introduce TAGPRIME to address relational structure extraction problems. TAGPRIME is a sequence tagging model that appends priming words about the information of the given condition (such as an event trigger) to the input text. With the self-attention mechanism in pre-trained language models, the priming words make the output contextualized representations contain more information about the given condition, and hence become more suitable for extracting specific relationships for the condition. Extensive experiments and analyses on three different tasks that cover ten datasets across five different languages demonstrate the generality and effectiveness of TAGPRIME.

==> 01-introduction_old.tex <==
\section{Introduction}
\label{sec:intro}
% what relational structure extraction is and why relational structure extraction is important
% Given a span as a condition, 
% relational structure extraction 

% relational structure extraction extracts the spans that maintain relationships or serve as attributes for the conditioned span, and on the same time, predicts their corresponding relations/attributes.

% Relational structure extraction identifies the span and the relationships/

% identifies the span that maintains a relationship with a given span and classifies the relationship.
Relational structure extraction aims to identify the arguments and classify the relationships regarding to a given span.
Many tasks in natural language processing require extracting relational structures from texts. For example, the event argument extraction task aims to identify event arguments and \textit{their corresponding roles for the given event trigger}~\cite{acl2022xgear, wang-etal-2019-hmeae}. 
In end-to-end relation extraction, the model identifies tail-entities and head-entities and recognizes \textit{their relationship}~\cite{DBLP:conf/acl/WeiSWTC20, DBLP:conf/ecai/0002ZSLWWL20}. 
In task-oriented semantic parsing, the model predicts the slots and \textit{their semantic roles for the given intent} in an utterance \cite{Tur10atis,Li21mtop}.
% \violet{it's not very obvious why would this be `relational'. relation between what?} \ihside{this better?}
These tasks are beneficial to a wide range of applications, such as dialog systems~\cite{liu2018knowledge}%, knowledge graph construction~\cite{DBLP:conf/www/ZhangLPSL20}
, question answering~\cite{yasunaga-etal-2021-qa}%,DBLP:conf/emnlp/HanHSBNRP21}
, and narrative generation~\cite{chen2019incorporating}.

\begin{figure*}[t!]
    \centering
    \includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=0.94\textwidth]{Figures/ACL2023_mthd_overview.pdf}
    \vspace{-0.3em}
    \caption{Illustrations of different models. 
    (a) \textbf{Graph-based method}: the node representation will be initialized through a pre-trained language model and be updated iteratively by aggregating possible neighbor nodes' information. 
    (b) \textbf{Sequence tagging model with conditional features}: A conventional sequence tagging model that embeds conditional information by adding learnable features to the output representation from a pre-trained language model. In the shown example, the conditional features contain two parts: one is the token embedding representing the conditional word \emph{``military''}, and the other is an entity type embedding. %for the \emph{``Organization''} type.
    (c) \textbf{\model{} with condition priming}: The conditional information is further applied to the input sequence to induce the output representation from the pre-trained language model to become condition-aware.
    (d) \textbf{\model{} with condition \& relationship priming}: Our approach that further append the verbalized relationship to \model{} with condition priming model. For this case, the goal of the tagging model is to make predictions specific to the relationship type in the input. \footnotemark}
    % Note that CRF layers in (b)\&(c)\&(d) are omitted for better readability.}
    \label{fig:mthd_overview}
    \vspace{-0.5em}
\end{figure*}


% many task specific methods for different task; graph-based work is one of the most commonly use framework to deal with such problems => edge prediction by feature concatenation and need iterative update to make node representation better suited for downstream tasks
Various task-specific methods have been proposed for different tasks that demand relational structure extraction. Graph-based methods are one of the most popular frameworks to deal with such problems \cite{DBLP:conf/naacl/LuanWHSOH19, Lin20oneie, DBLP:conf/acl/SunGWGJLSD19, DBLP:conf/acl/MiwaB16, DBLP:conf/acl/FuLM19}. 
These methods extract relational structures by repeatedly constructing graphs and updating span representations, as illustrated in Figure~\ref{fig:mthd_overview}(a).
% By leveraging the relational interaction between spans in the constructed graph, the models iteratively update the span representations in the sentence, 
% \kh{We need talk more about why they choose complex graph-based models.}
The graph enables models to incorporate potential relational structure and aggregate information in a non-local manner. Hence, the updated span representations become more comprehensive and better suited for the relational extraction tasks. %modeling the whole graph structure,



% tagging model is a conventional method to deal with relational structure extraction in general. for a long time, it's less emphasized as graph-based model xxx. using priming => task-specific => more suitable for capturing relational structure. => become a strong baseline
On the other hand, sequence tagging models are conventional methods for relational structure extraction~\cite{DBLP:conf/acl/YangFQKL19, DBLP:conf/interspeech/Hakkani-TurTCCG16, DBLP:conf/emnlp/MaWABA20, DBLP:conf/icann/ZhangFCLCT18, DBLP:conf/emnlp/RamponiGLP20}.
Tagging models convert the relational structure into a sequential format and make predictions by sequentially labeling tokens in the input passage.
To address the information required for prediction (such as the given span's properties), sequence tagging models usually incorporate learnable feature embeddings before the tags are assigned, as illustrated in Figure~\ref{fig:mthd_overview}(b). Compared to graph-based models, recently tagging models get less attention in the research community due to their simplicity.
%since graph-based methods, in theory, capture more complex interactions between spans and thus lead to stronger results.

% emphasize unified more, less detail
In this work, we re-examine the effectiveness of sequence tagging methods on relational structure extraction and present \model{}, a simple, unified, yet strong model. 
Inspired by \citet{DBLP:journals/corr/abs-2109-12383}, we introduce \emph{priming technique} to sequence tagging models, which augments the input text with task-specific contexts, 
% and performs sequence tagging on the input text, 
as illustrated in Figure~\ref{fig:mthd_overview}(c) \& (d).
With the self-attention mechanism in pre-trained language models, the priming approach %exploits the nature of contextualized pre-trained language models and 
makes the sentence representations \emph{task-specific} directly. Thus, it unlocks the capability of sequence tagging methods for relational structure extraction better than the commonly used feature embedding approach, as will be shown in Section~\ref{sec:analysis}.

We conduct thorough experiments to evaluate \model{} on three different tasks (end-to-end event extraction, end-to-end relation extraction, and task-oriented semantic parsing). The experiments cover ten datasets in five different languages. We show that \model{} achieves comparable or better performance than the current state-of-the-art models on almost all the datasets.
Hence, we suggest that \model{} can serve as a strong baseline for future studies. Additionally, we perform comprehensive ablation studies to understand the underlying merits of \model{}, and present analysis to the inference speed of \model{}.
\footnotetext{We omit CRF layers in Figure~\ref{fig:mthd_overview} (b)(c)(d) for readability.}

% we perform analysis to study the layer sharing for priming method. base on our study, xxx can be more efficient.
% \violet{I commented out the following paragraph as I don't think it's that important to discuss in the intro.}
% In addition, to better understand the mechanism of priming, we carry out experiments to analyze whether deeply-stacked layers is essential for priming method to equip the sentential representation with task-specific information. 
% We observe that although deeper layers help, priming sequential models with much shallower layers can achieve similar performance. Based on the study, we further introduce an efficient approximation of the sequential tagging model with priming and the approximating model can achieve similar performance but faster inference speed.

% contribution: (1) a unified model with baseline (2) analysis
% Our contributions can be summarized as follows. 
% (1) We present \model{}, a simple and unified sequence tagging model that can tackle several relational structure extraction tasks and serve as a strong baseline for further studies. 
% (2) \model{} achieves comparable or better performance than the current state-of-the-art on three different tasks across various languages.
% The model is verified in three different tasks and in various languages. The results are comparable or achieve a new state-of-the-art on three different natural language processing tasks in ten datasets in total. 
% (3) We perform a thorough analysis on the priming methods, and propose a novel efficient approximation to fasten up models during inference time with only a small performance drop. \violet{I'll move the discussion about the speedup to be under (1).}

==> 02-background.tex <==
\section{Relational Structure Extraction}
\label{sec:background}
In this work, we focus on relational structure extraction, which can be applied to many natural language processing tasks.
For example, pipelined approaches to end-to-end event extraction involve
extracting event arguments and their corresponding roles for the given event trigger \ih{(cite)}.
The subtask in task-oriented semantic parsing, slot filling, predicts the slots and the semantic roles in the utterance for the given intent \ih{(cite)}.
Some recent works tackle end-to-end relation extraction by adopting a cascading pipeline such that after head-entities are first identified, a model will jointly predict tail-entities and their relation for each head-entity~\cite{DBLP:conf/acl/WeiSWTC20, DBLP:conf/ecai/0002ZSLWWL20, DBLP:conf/acl/SunGWGJLSD19}.
These methods on different tasks all consists of a procedure that extracts a relational structure conditioned on a given object, and we take a unified view to these procedures and form the task --- relational structure extraction.

More formally, given an input passage and a condition $\mbf c$, a relational structure extraction model identifies a list of objects $\mbf o^c = [o^c_1, o^c_2, ..., o^c_l]$ and their corresponding relation $\mbf r^c = [r^c_1, r^c_2, ..., r^c_l]$ for the condition $\mbf c$. For instance, the given trigger, intent, and head-entity are the conditions for the aforementioned tasks, and the goals to extract are the event arguments (with their argument roles), slots (with their semantic roles), and tail-entities (with their relationships toward the head-entity).
